Precision measurement of CP violation and branching fractions in $B^{\pm} \to K^0_{\mathrm{S}} h^{\pm}$ $(h = \pi, K)$ decays and search for the rare decay $B_c^{\pm} \to K^0_{\mathrm{S}} K^{\pm}$

The decay $B^{\pm} \to K^0_{\mathrm{S}} \pi^{\pm}$, with a $CP$ asymmetry expected to be close to zero in the Standard Model, is theoretically clean and sensitive to potential new physics. An analysis of the decays $B^{\pm} \to K^0_{\mathrm{S}} \pi^{\pm}$ and $B^{\pm} \to K^0_{\mathrm{S}} K^{\pm}$ is performed using proton-proton collision data collected by the LHCb experiment at a center-of-mass energy of $13\,\mathrm{TeV}$, corresponding to an integrated luminosity of $5.4\,\mathrm{fb}^{-1}$. The \CP asymmetries are determined to be ${\cal A}^{CP}(B^{\pm} \to K^0_{\mathrm{S}} \pi^{\pm})=-0.028\pm 0.009\pm 0.009$ and ${\cal A}^{CP}(B^{\pm} \to K^0_{\mathrm{S}} K^{\pm})=0.118\pm 0.062 \pm 0.031$, and the branching fraction ratio is measured to be ${\cal B}(B^{\pm} \to K^0_{\mathrm{S}} K^{\pm})/{\cal B}(B^{\pm} \to K^0_{\mathrm{S}} \pi^{\pm})=0.055\pm 0.004 \pm 0.002$, where the first uncertainties are statistical and the second are systematic. These results are the most precise measurements of these quantities to date. A search for the rare decay $B_c^{\pm} \to K^0_{\mathrm{S}} K^{\pm}$ is also performed. No significant signal is observed, and the upper limit on the product of the branching fraction ratio ${\cal B}(B_c^{\pm} \to K^0_{\mathrm{S}} K^{\pm})/{\cal B}(B^{\pm} \to K^0_{\mathrm{S}} \pi^{\pm})$ and the fragmentation-fraction ratio $f_c/f_u$ is set to be 0.015 (0.016) at the 90\% (95\%) confidence level.

==> Authorship_LHCb-PAPER-2025-049-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin\'en,
T. Ackernley,
A.A. Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
M. Akthar,
P. Albicocco,
J. Albrecht,
R. Aleksiejunas,
F. Alessio,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
P. Andreola,
M. Andreotti,
S. Andres Estrada,
A. Anelli,
D. Ao,
C. Arata,
F. Archilli,
Z. Areg,
M. Argenton,
S. Arguedas Cuendis,
L. Arnone,
A. Artamonov,
M. Artuso,
E. Aslanides,
R. Ata\'ide Da Silva,
M. Atzeni,
B. Audurier,
J.A. Authier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
A. Balboni,
W. Baldini,
Z. Baldwin,
L. Balzani,
H. Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I.R. Barbosa,
R.J. Barlow,
M. Barnyakov,
S. Barsuk,
W. Barter,
J. Bartz,
S. Bashir,
B. Batsukh,
P.B. Battista,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N.A. Behling,
S. Belin,
A. Bellavista,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
A. Bertolin,
F. Betti,
J. Bex,
O. Bezshyyko,
S. Bhattacharya,
M.S. Bieker,
N.V. Biesuz,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Bohare,
A. Boldyrev,
C. Bolognani,
R. Bolzonella,
R.B. Bonacci,
N. Bondar,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E. Bottalico,
S.A. Bouchiba,
M. Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J.D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
J. Brown,
D. Brundu,
E. Buchanan,
M. Burgos Marcos,
A.T. Burke,
C. Burr,
C. Buti,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
Y. Cai,
A. Caillet,
R. Calabrese,
S. Calderon Ramirez,
L. Calefice,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J.I. Cambon Bouzas,
P. Campana,
A.F. Campoverde Quezada,
Y. Cao,
S. Capelli,
M. Caporale,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
I. Celestino,
S. Cesare,
A.J. Chadwick,
I. Chahrour,
H. Chang,
M. Charles,
Ph. Charpentier,
E. Chatzianagnostou,
R. Cheaib,
M. Chefdeville,
C. Chen,
J. Chen,
S. Chen,
Z. Chen,
A. Chen Hu,
M. Cherif,
A. Chernov,
S. Chernyshenko,
X. Chiotopoulos,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S. Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
J. Connaughton,
A. Contu,
N. Cooke,
G. Cordova,
C. Coronel,
I. Corredoira ,
A. Correia,
G. Corti,
J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
M. Cubero Campos,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
G. Darze,
A. Davidson,
J.E. Davies,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
S. Dekkers,
L. Del Buono,
B. Delaney,
J. Deng,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
Y. Ding,
L. Dittmann,
V. Dobishuk,
A.D. Docheva,
A. Doheny,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
A.D. Dowling,
L. Dreyfus,
W. Duan,
P. Duda,
L. Dufour,
V. Duk,
P. Durante,
M.M. Duras,
J.M. Durham,
O.D. Durmus,
A. Dziurda,
A. Dzyuba,
S. Easo,
E. Eckstein,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
D. Elizondo Blanco,
J. Ellbracht,
S. Ely,
A. Ene,
J. Eschle,
T. Evans,
F. Fabiano,
S. Faghih,
L.N. Falcao,
B. Fang,
R. Fantechi,
L. Fantini,
M. Faria,
K. Farmer,
F. Fassin,
D. Fazzini,
L. Felkowski,
C. Feng,
M. Feng,
A. Fernandez Casani,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.L. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
A. Fomin,
M. Fontana,
L.A. Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. F\"uhring,
T. Fulghesu,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B. Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc\'ia Pardi\~nas,
P. Gardner,
L. Garrido,
C. Gaspar,
A. Gavrikov,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
F.I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent\`u,
L. Girardey,
M.A. Giza,
F.C. Glaser,
V.V. Gligorov,
C. G\"obel,
L. Golinka-Bezshyyko,
E. Golobardes,
D. Golubkov,
A. Golutvin,
S. Gomez Fernandez,
W. Gomulka,
F. Goncalves Abrantes,
I. Gon\c{c}ales Vaz,
M. Goncerz,
G. Gong,
J.A. Gooding,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug\'es,
E. Graverini,
L. Grazette,
G. Graziani,
A.T. Grecu,
N.A. Grieser,
L. Grillo,
S. Gromov,
C. Gu,
M. Guarise,
L. Guerry,
A.-K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S. Haken,
G. Hallett,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
T.J. Harris,
M. Hartmann,
S. Hashmi,
J. He,
N. Heatley,
A. Hedes,
F. Hemmer,
C. Henderson,
R. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A. Heyn,
A. Hicheur,
G. Hijano Mendizabal,
J. Horswill,
R. Hou,
Y. Hou,
D.C. Houston,
N. Howarth,
W. Hu,
X. Hu,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
M. Idzik,
D. Ilin,
P. Ilten,
A. Iniukhin,
A. Iohner,
A. Ishteev,
K. Ivshin,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
T. Jakoubek,
E. Jans,
B.K. Jashal,
A. Jawahery,
C. Jayaweera,
V. Jevtic,
Z. Jia,
E. Jiang,
X. Jiang,
Y. Jiang,
Y.J. Jiang,
E. Jimenez Moya,
N. Jindal,
M. John,
A. John Rubesh Rajan,
D. Johnson,
C.R. Jones,
S. Joshi,
B. Jost,
J. Juan Castella,
N. Jurik,
I. Juszczak,
K. Kalecinska,
D. Kaminaris,
S. Kandybei,
M. Kane,
Y. Kang,
C. Kar,
M. Karacson,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
T. Kirn,
V.S. Kirsebom,
S. Klaver,
N. Kleijne,
A. Kleimenova,
D.K. Klekots,
K. Klimaszewski,
M.R. Kmiec,
T. Knospe,
R. Kolb,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
A. Korchin,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
E. Kowalczyk,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
O. Kravcov,
M. Kreps,
P. Krokovny,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
V. Kushnir,
B. Kutsenko,
J. Kvapil,
I. Kyryllin,
D. Lacarrere,
P. Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H. Lee,
R. Lef\`evre,
A. Leflat,
S. Legotin,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E.D. Lesser,
B. Leverington,
A. Li,
C. Li,
C. Li,
H. Li,
J. Li,
K. Li,
L. Li,
M. Li,
P. Li,
P.-R. Li,
Q. Li,
T. Li,
T. Li,
Y. Li,
Y. Li,
Y. Li,
Z. Lian,
Q. Liang,
X. Liang,
Z. Liang,
S. Libralon,
A. Lightbody,
C. Lin,
T. Lin,
R. Lindner,
H. Linton,
R. Litvinov,
D. Liu,
F.L. Liu,
G. Liu,
K. Liu,
S. Liu,
W. Liu,
Y. Liu,
Y. Liu,
Y.L. Liu,
G. Loachamin Ordonez,
I. Lobo,
A. Lobo Salvia,
A. Loi,
T. Long,
F.C.L. Lopes,
J.H. Lopes,
A. Lopez Huertas,
C. Lopez Iribarnegaray,
S. L\'opez Soli\~no,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
S. Lyu,
X.-R. Lyu,
G.M. Ma,
H. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B. Mack,
I. Mackay,
L.M. Mackey,
L.R. Madhan Mohan,
M.J. Madurai,
D. Magdalinski,
D. Maisuzenko,
J.J. Malczewski,
S. Malde,
L. Malentacca,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
F.M. Manganella,
D. Manuzzi,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L. Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A. Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
M. McCann,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
D. Melnychuk,
D. Mendoza Granada,
P. Menendez Valdes Perez,
F.M. Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
T. Miralles,
B. Mitreska,
D.S. Mitzel,
R. Mocanu,
A. Modak,
L. Moeser,
R.D. Moise,
E.F. Molina Cardenas,
T. Momb\"acher,
M. Monk,
T. Monnard,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A. Moro,
J. Moron,
W. Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
Z. Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M\"uller,
F. Mu\~noz-Rojas,
R. Murta,
V. Mytrochenko,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
G. Napoletano,
I. Nasteva,
M. Needham,
E. Nekrasova,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
J. Nicolini,
D. Nicotra,
E.M. Niel,
N. Nikitin,
L. Nisi,
Q. Niu,
B.K. Njoki,
P. Nogarolli,
P. Nogga,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
H.N. Nur,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
A. Okhotnikov,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
E. Olivart Pino,
M. Olocco,
R.H. O'Neil,
J.S. Ordonez Soto,
D. Osthues,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A. Padee,
K.O. Padeken,
B. Pagare,
T. Pajero,
A. Palano,
L. Palini,
M. Palutan,
C. Pan,
X. Pan,
S. Panebianco,
S. Paniskaki,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D. Parmar,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A. Paul,
C.J. Pawley,
A. Pellegrino,
J. Peng,
X. Peng,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
H. Pereira Da Costa,
M. Pereira Martinez,
A. Pereiro Castro,
C. Perez,
P. Perret,
A. Perrevoort,
A. Perro,
M.J. Peters,
K. Petridis,
A. Petrolini,
S. Pezzulo,
J.P. Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L. Piccolo,
B. Pietrzyk,
G. Pietrzyk,
R.N. Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V.M. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
K. Popp,
S. Poslavskii,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
A. Puicercus Gomez,
G. Punzi,
J.R. Pybus,
Q. Qian,
W. Qian,
N. Qin,
R. Quagliani,
R.I. Rabadan Trejo,
R. Racz,
J.H. Rademacker,
M. Rama,
M. Ram\'irez Garc\'ia,
V. Ramos De Oliveira,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
M. Ribalda Galvez,
R. Ribatti,
G. Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
F. Riehn,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogachev,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
M. Rotondo,
S.R. Roy,
M.S. Rudolph,
M. Ruiz Diaz,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
J.J. Saavedra-Arias,
J.J. Saborido Silva,
S.E.R. Sacha Emile R.,
N. Sagidova,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
D. Saranin,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
F. Sborzacchi,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
N. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
M.H. Schune,
G. Schwering,
B. Sciascia,
A. Sciuccati,
G. Scriven,
I. Segal,
S. Sellam,
A. Semennikov,
T. Senger,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
B. Sevilla Sanjuan,
Y. Shang,
D.M. Shangase,
M. Shapkin,
R.S. Sharma,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
J. Shen,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
Q. Shi,
W.S. Shi,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
J.D. Shupperd,
R. Silva Coutinho,
G. Simi,
S. Simone,
M. Singha,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
E. Smith,
M. Smith,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
K. Solovieva,
N.S. Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y.S. Song,
F.L. Souza De Almeida,
B. Souza De Paula,
K.M. Sowa,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
M. Stefaniak,
O. Steinkamp,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
J. Sun,
L. Sun,
D. Sundfeld,
W. Sutcliffe,
P. Svihra,
V. Svintozelskyi,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
Y.T. Tang,
M.D. Tat,
J.A. Teijeiro Jimenez,
A. Terentev,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
A.R. Thomson-Strong,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
T.T. Todorov,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
D.J. Unverzagt,
A. Upadhyay,
B. Urbach,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
A. Vaitkevicius,
V. Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
G. Vasquez,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V\'azquez Sierra,
S. Vecchi,
J. Velilla Serna,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
W. Vetens,
D. Vico Benet,
P. Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
B. Vivacqua,
F.C. Volle,
D. vom Bruch,
N. Voropaev,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
E.J. Walton,
G. Wan,
A. Wang,
B. Wang,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N.W. Wang,
R. Wang,
X. Wang,
X. Wang,
X.W. Wang,
Y. Wang,
Y. Wang,
Y.H. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
Z. Weida,
J. Wendel,
B.D.C. Westhenry,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
M.A. Wiegertjes,
C. Wild,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M.J. Williams,
M.R.J. Williams,
R. Williams,
S. Williams,
Z. Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
T. Wolf,
E. Wood,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T.X. Xing,
A. Xu,
L. Xu,
M. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
S. Yadav,
K. Yang,
X. Yang,
Y. Yang,
Y. Yang,
Z. Yang,
V. Yeroshenko,
H. Yeung,
H. Yin,
X. Yin,
C.Y. Yu,
J. Yu,
X. Yuan,
Y Yuan,
J.A. Zamora Saa,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C. Zeng,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
R. Zhang,
S. Zhang,
S.L. Zhang,
Y. Zhang,
Y.Z. Zhang,
Z. Zhang,
Y. Zhao,
A. Zhelezov,
S.Z. Zheng,
X.Z. Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
L.Z. Zhu,
X. Zhu,
X. Zhu,
Y. Zhu,
V. Zhukov,
J. Zhuo,
D. Zuliani,
G. Zunica
